Learning to Break: Knowledge-Enhanced Reasoning in Multi-Agent Debate System

Multi-agent debate system (MAD) imitating the process of human discussion in pursuit of truth, aims to align the correct cognition of different agents for the optimal solution. It is challenging to make various agents perform right and highly consistent cognition due to their limited and different knowledge backgrounds (i.e., cognitive islands), which hinders the search for the optimal solution. To address the challenge, we propose a novel \underline{M}ulti-\underline{A}gent \underline{D}ebate with \underline{K}nowledge-\underline{E}nhanced framework (\textbf{MADKE}) to promote the system to find the solution. First, we involve a shared retrieval knowledge pool in the debate process to solve the problem of limited and different knowledge backgrounds. Then, we propose an adaptive knowledge selection method to guarantee the accuracy and personalization of knowledge. This method allows agents to choose whether to use external knowledge in each conversation round according to their own needs. Our experimental results on six datasets show that our method achieves state-of-the-art results compared to existing single-agent and multi-agent methods. Further analysis reveals that the introduction of retrieval knowledge can help the agent to break cognitive islands in the debate process and effectively improve the consistency and correctness of the model. Moreover, MADKE using Qwen1.5-72B-Chat surpasses GPT-4 by +1.26\% on average in six datasets, which validates that our method can help open-source LLMs achieve or even surpass the performance of GPT-4. Our code is available at \url{https://github.com/FutureForMe/MADKE}.

==> sections/acknowledgements.tex <==
\section*{Acknowledgements}
% This work is supported in part by the National Natural Science Foundation of China [grant number 62141201], Natural Science Foundation of Chongqing [grant number CSTB2022NSCQ-MSX1672]. 

This work is supported in part by the National Key R\&D Program of China [2021ZD0113302] and  National Key R\&D Program of China [2021ZD0110900]. We thank all the anonymous reviewers for generously contributing their time and effort. Their professional advice greatly improved the quality of the manuscript.

% 这项工作得到了科技部项目【】的部分支持。我们感谢所有的匿名审稿人慷慨地贡献了他们的时间和精力。他们的专业建议大大提高了稿件的质量。

==> sections/limitations.tex <==
\section*{Limitations}
Compared with a single agent, our method requires repeated calls to the model to generate content, which results in higher generation costs. However, we believe that this approach is necessary because it can alleviate the illusion of large models, solve the cognitive islands of the debate process, and effectively promote the implementation of large models. 
